Contagion Effects of the Silicon Valley Bank Run

This paper analyzes the contagion effects associated with the failure of Silicon Valley Bank (SVB) and identifies bank-specific vulnerabilities contributing to the subsequent declines in banks' stock returns. We find that uninsured deposits, unrealized losses in held-to-maturity securities, bank size, and cash holdings had a significant impact, while better-quality assets or holdings of liquid securities did not help mitigate the negative spillovers. Interestingly, banks whose stocks performed worse post-SVB also experienced lower returns in the previous year, following Federal Reserve interest rate hikes. Stock investors appeared to anticipate risks associated with uninsured deposit reliance, but did not foresee the realization of implied losses. While mid-sized banks experienced particular stress immediately after the SVB failure, over time negative spillovers became widespread except for the largest banks.

==> figures/table1_y9c.tex <==
\begin{table}[!htbp] \centering \renewcommand*{\arraystretch}{1.1}\caption{Summary Statistics}\resizebox{\textwidth}{!}{
\begin{tabular}{lrrrr}
\hline
\hline
Variable & NotNA & Mean & Median & Sd \\ 
\hline
Assets (000) & 224 & 101688402 & 9559211 & 405,970,115 \\ 
Cash / Assets & 224 & 9.2\% & 8.1\% & 7\% \\ 
Securities / Assets & 224 & 20\% & 18\% & 11\% \\ 
Liquid Assets / Assets & 224 & 29\% & 27\% & 13\% \\ 
Unrealized HTM Losses / Tier 1 Capital & 222 & 0.21\% & 0\% & 2.2\% \\ 
Hold-to-Maturity Securities / Assets & 224 & 3.2\% & 0.33\% & 5.9\% \\ 
Unisured Deposit Share & 224 & 39\% & 38\% & 18\% \\ 
Tier 1 Capital Ratio & 216 & 13\% & 12\% & 2.9\%\\ 
\hline
\hline
\end{tabular}
}
\end{table}



==> figures/table2.tex <==
\begin{table}[!htbp] \centering \renewcommand*{\arraystretch}{1.1}\caption{Summary Statistics}\resizebox{\textwidth}{!}{
\begin{tabular}{lrrrrrrr}
\hline
\hline
Variable & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{SD} & \multicolumn{1}{c}{5th Pct.} & \multicolumn{1}{c}{25th Pct.} & \multicolumn{1}{c}{50th Pct.} & \multicolumn{1}{c}{75th Pct.} & \multicolumn{1}{c}{95th Pct.} \\ 
\hline
\multicolumn{8}{c}{Date: 2023-01-31} \\ 
Cumulative Abnormal Returns & 2.9\% & 15\% & -25\% & -5.7\% & 3.7\% & 12\% & 27\% \\ 
 &  &  &  &  &  &  &  \\ 
\multicolumn{8}{c}{Date: 2023-03-17} \\ 
Cumulative Abnormal Returns & -16\% & 13\% & -35\% & -18\% & -14\% & -8.2\% & -2.6\% \\ 
 &  &  &  &  &  &  &  \\ 
\multicolumn{8}{c}{Date: 2023-05-10} \\ 
Cumulative Abnormal Returns & -34\% & 16\% & -57\% & -41\% & -33\% & -24\% & -12\%\\ 
\hline
\hline
\end{tabular}
}
\end{table}



==> figures/table3.tex <==

\begin{table}[htbp]
   \caption{\label{tab:dep_htm} Cumulative returns correlated with uninsured deposits and HTM. This table reports estimated coefficients of regressions with the cumulative returns in excess of the S\&P 500 index for the banks in our sample from February 1, 2023 to March 17, 2023 as the outcome.  In Column (1), we report the bivariate relationship with the uninsured deposit share (uninsured deposts as a share of total
   deposits) measured in 2022q4. Column (2) reports the coefficient with the hold-to-maturity asset share (hold-to-maturity assets
   as a share of total assets) measured in 2022q4. Column (3) reports unrealized hold-to-
   maturity losses scaled by tier 1 capital. Column (4) combines Columns (1)-(3). Column (5) adds the interaction of uninsured deposit share with HTM Asset Share and Unrealized HTM Losses. All variables (except for the cumulative returns) are mean zero and standarized to have standard deviation one, prior to interactions.}
   \bigskip
   \centering
   \begin{adjustbox}{width = 1.2\textwidth, center}
      \begin{tabular}{lccccc}
         \toprule
                                                                                  & (1)            & (2)            & (3)            & (4)            & (5)\\  
         \midrule 
         (Intercept)                                                              & -0.156$^{***}$ & -0.156$^{***}$ & -0.156$^{***}$ & -0.156$^{***}$ & -0.145$^{***}$\\   
                                                                                  & (0.008)        & (0.008)        & (0.008)        & (0.007)        & (0.007)\\   
         Uninsured Deposit Share                                                  & -0.048$^{***}$ &                &                & -0.035$^{***}$ & -0.030$^{***}$\\   
                                                                                  & (0.015)        &                &                & (0.011)        & (0.009)\\   
         HTM Asset Share                                                          &                & -0.046$^{**}$  &                & -0.020         & -0.008\\   
                                                                                  &                & (0.018)        &                & (0.015)        & (0.007)\\   
         Unrealized HTM Losses / Tier 1 Capital                                   &                &                & -0.062$^{***}$ & -0.048$^{***}$ & 0.007\\   
                                                                                  &                &                & (0.014)        & (0.009)        & (0.018)\\   
         Uninsured Deposit Share $\times$ HTM Asset Share                         &                &                &                &                & -0.008\\   
                                                                                  &                &                &                &                & (0.008)\\   
         Uninsured Deposit Share $\times$ Unrealized HTM Losses / Tier 1 Capital  &                &                &                &                & -0.040$^{***}$\\   
                                                                                  &                &                &                &                & (0.015)\\   
          \\
         Observations                                                             & 224            & 224            & 222            & 222            & 222\\  
         R$^2$                                                                    & 0.139          & 0.124          & 0.224          & 0.328          & 0.420\\  
         Adjusted R$^2$                                                           & 0.135          & 0.120          & 0.221          & 0.318          & 0.406\\  
         \bottomrule
      \end{tabular}
   \end{adjustbox}
\end{table}




==> figures/table3_beta.tex <==

\begin{table}[htbp]
   \caption{\label{tab:dep_htm_beta} Cumulative returns correlated with uninsured deposits and HTM, adjusted for beta. This table reports estimated coefficients of regressions with the cumulative returns in excess of the S\&P 500 index, adjusting for beta estimated in 2022, for the banks in our sample from February 1, 2023 to March 17, 2023 as the outcome.  In Column (1), we report the bivariate relationship with the uninsured deposit share (uninsured deposts as a share of total deposits) measured in 2022q4. Column (2) reports the coefficient with the hold-to-maturity asset share (hold-to-maturity assets as a share of total assets) measured in 2022q4. Column (3) reports unrealized hold-to-maturity losses scaled by tier 1 capital. Column (4) combines Columns (1)-(3). Column (5) adds the interaction of uninsured deposit share with HTM Asset Share and Unrealized HTM Losses. All variables (except for the cumulative returns) are mean zero and standarized to have standard deviation one, prior to interactions.}
   \bigskip
   \centering
   \begin{adjustbox}{width = 1.2\textwidth, center}
      \begin{tabular}{lccccc}
         \toprule
                                                                                  & (1)            & (2)            & (3)            & (4)            & (5)\\  
         \midrule 
         (Intercept)                                                              & -0.165$^{***}$ & -0.165$^{***}$ & -0.166$^{***}$ & -0.166$^{***}$ & -0.154$^{***}$\\   
                                                                                  & (0.008)        & (0.008)        & (0.008)        & (0.007)        & (0.007)\\   
         Uninsured Deposit Share                                                  & -0.048$^{***}$ &                &                & -0.034$^{***}$ & -0.029$^{***}$\\   
                                                                                  & (0.016)        &                &                & (0.011)        & (0.010)\\   
         HTM Asset Share                                                          &                & -0.046$^{**}$  &                & -0.020         & -0.007\\   
                                                                                  &                & (0.018)        &                & (0.016)        & (0.007)\\   
         Unrealized HTM Losses / Tier 1 Capital                                   &                &                & -0.063$^{***}$ & -0.049$^{***}$ & 0.007\\   
                                                                                  &                &                & (0.015)        & (0.009)        & (0.018)\\   
         Uninsured Deposit Share $\times$ HTM Asset Share                         &                &                &                &                & -0.009\\   
                                                                                  &                &                &                &                & (0.008)\\   
         Uninsured Deposit Share $\times$ Unrealized HTM Losses / Tier 1 Capital  &                &                &                &                & -0.042$^{***}$\\   
                                                                                  &                &                &                &                & (0.016)\\   
          \\
         Observations                                                             & 224            & 224            & 222            & 222            & 222\\  
         R$^2$                                                                    & 0.136          & 0.125          & 0.233          & 0.332          & 0.430\\  
         Adjusted R$^2$                                                           & 0.132          & 0.121          & 0.230          & 0.323          & 0.417\\  
         \bottomrule
      \end{tabular}
   \end{adjustbox}
\end{table}




==> figures/table3_late.tex <==

\begin{table}[htbp]
   \caption{\label{tab:dep_htm_late} Cumulative returns correlated with uninsured deposits and HTM, long run. This table reports estimated coefficients of regressions with the cumulative returns in excess of the S\&P 500 index, adjusting for beta estimated in 2022, for the banks in our sample from February 1, 2023 to May 10, 2023 as the outcome.  In Column (1), we report the bivariate relationship with the uninsured deposit share (uninsured deposts as a share of total deposits) measured in 2022q4. Column (2) reports the coefficient with the hold-to-maturity asset share (hold-to-maturity assets as a share of total assets) measured in 2022q4. Column (3) reports unrealized hold-to-maturity losses scaled by tier 1 capital. Column (4) combines Columns (1)-(3). Column (5) adds the interaction of uninsured deposit share with HTM Asset Share and Unrealized HTM Losses. All variables (except for the cumulative returns) are mean zero and standarized to have standard deviation one, prior to interactions.}
   \bigskip
   \centering
   \begin{adjustbox}{width = 1.2\textwidth, center}
      \begin{tabular}{lccccc}
         \toprule
                                                                                  & (1)            & (2)            & (3)            & (4)            & (5)\\  
         \midrule 
         (Intercept)                                                              & -0.336$^{***}$ & -0.336$^{***}$ & -0.338$^{***}$ & -0.338$^{***}$ & -0.325$^{***}$\\   
                                                                                  & (0.010)        & (0.011)        & (0.010)        & (0.010)        & (0.010)\\   
         Uninsured Deposit Share                                                  & -0.051$^{***}$ &                &                & -0.044$^{***}$ & -0.040$^{***}$\\   
                                                                                  & (0.016)        &                &                & (0.013)        & (0.011)\\   
         HTM Asset Share                                                          &                & -0.037$^{**}$  &                & -0.010         & -0.005\\   
                                                                                  &                & (0.018)        &                & (0.015)        & (0.012)\\   
         Unrealized HTM Losses / Tier 1 Capital                                   &                &                & -0.052$^{***}$ & -0.039$^{***}$ & 0.036$^{**}$\\   
                                                                                  &                &                & (0.012)        & (0.011)        & (0.015)\\   
         Uninsured Deposit Share $\times$ HTM Asset Share                         &                &                &                &                & 0.0004\\   
                                                                                  &                &                &                &                & (0.008)\\   
         Uninsured Deposit Share $\times$ Unrealized HTM Losses / Tier 1 Capital  &                &                &                &                & -0.057$^{***}$\\   
                                                                                  &                &                &                &                & (0.011)\\   
          \\
         Observations                                                             & 224            & 224            & 222            & 222            & 222\\  
         R$^2$                                                                    & 0.097          & 0.052          & 0.103          & 0.181          & 0.269\\  
         Adjusted R$^2$                                                           & 0.093          & 0.048          & 0.099          & 0.170          & 0.252\\  
         \bottomrule
      \end{tabular}
   \end{adjustbox}
\end{table}




==> figures/table3_late_beta.tex <==

\begin{table}[htbp]
   \caption{\label{tab:dep_htm_late_beta} Cumulative returns correlated with uninsured deposits and HTM, long run and adjusted for beta. This table reports estimated coefficients of regressions with the cumulative returns in excess of the S\&P 500 index for the banks in our sample from February 1, 2023 to May 10, 2023 as the outcome.  In Column (1), we report the bivariate relationship with the uninsured deposit share (uninsured deposts as a share of total deposits) measured in 2022q4. Column (2) reports the coefficient with the hold-to-maturity asset share (hold-to-maturity assets as a share of total assets) measured in 2022q4. Column (3) reports unrealized hold-to-maturity losses scaled by tier 1 capital. Column (4) combines Columns (1)-(3). Column (5) adds the interaction of uninsured deposit share with HTM Asset Share and Unrealized HTM Losses. All variables (except for the cumulative returns) are mean zero and standarized to have standard deviation one, prior to interactions.}
   \bigskip
   \centering
   \begin{adjustbox}{width = 1.2\textwidth, center}
      \begin{tabular}{lccccc}
         \toprule
                                                                                  & (1)            & (2)            & (3)            & (4)            & (5)\\  
         \midrule 
         (Intercept)                                                              & -0.321$^{***}$ & -0.321$^{***}$ & -0.323$^{***}$ & -0.323$^{***}$ & -0.310$^{***}$\\   
                                                                                  & (0.010)        & (0.011)        & (0.010)        & (0.010)        & (0.010)\\   
         Uninsured Deposit Share                                                  & -0.050$^{***}$ &                &                & -0.044$^{***}$ & -0.040$^{***}$\\   
                                                                                  & (0.016)        &                &                & (0.013)        & (0.011)\\   
         HTM Asset Share                                                          &                & -0.037$^{**}$  &                & -0.010         & -0.005\\   
                                                                                  &                & (0.017)        &                & (0.015)        & (0.011)\\   
         Unrealized HTM Losses / Tier 1 Capital                                   &                &                & -0.052$^{***}$ & -0.039$^{***}$ & 0.036$^{**}$\\   
                                                                                  &                &                & (0.012)        & (0.011)        & (0.015)\\   
         Uninsured Deposit Share $\times$ HTM Asset Share                         &                &                &                &                & 0.0006\\   
                                                                                  &                &                &                &                & (0.008)\\   
         Uninsured Deposit Share $\times$ Unrealized HTM Losses / Tier 1 Capital  &                &                &                &                & -0.057$^{***}$\\   
                                                                                  &                &                &                &                & (0.010)\\   
          \\
         Observations                                                             & 224            & 224            & 222            & 222            & 222\\  
         R$^2$                                                                    & 0.097          & 0.052          & 0.104          & 0.182          & 0.270\\  
         Adjusted R$^2$                                                           & 0.093          & 0.048          & 0.100          & 0.171          & 0.253\\  
         \bottomrule
      \end{tabular}
   \end{adjustbox}
\end{table}




==> figures/table3_short.tex <==

\begin{table}[htbp]
   \caption{\label{tab:dep_htm_short} Cumulative returns correlated with uninsured deposits and HTM, immediately after SVB shutdown. This table reports estimated coefficients of regressions with the cumulative returns in excess of the S\&P 500 index for the banks in our sample from February 1, 2023 to March 10, 2023 as the outcome.  In Column (1), we report the bivariate relationship with the uninsured deposit share (uninsured deposts as a share of total
   deposits) measured in 2022q4. Column (2) reports the coefficient with the hold-to-maturity asset share (hold-to-maturity assets
   as a share of total assets) measured in 2022q4. Column (3) reports unrealized hold-to-
   maturity losses scaled by tier 1 capital. Column (4) combines Columns (1)-(3). Column (5) adds the interaction of uninsured deposit share with HTM Asset Share and Unrealized HTM Losses. All variables (except for the cumulative returns) are mean zero and standarized to have standard deviation one, prior to interactions.}
   \bigskip
   \centering
   \begin{adjustbox}{width = 1.2\textwidth, center}
      \begin{tabular}{lccccc}
         \toprule
                                                                                  & (1)            & (2)            & (3)            & (4)            & (5)\\  
         \midrule 
         (Intercept)                                                              & -0.071$^{***}$ & -0.071$^{***}$ & -0.071$^{***}$ & -0.071$^{***}$ & -0.061$^{***}$\\   
                                                                                  & (0.006)        & (0.006)        & (0.006)        & (0.005)        & (0.005)\\   
         Uninsured Deposit Share                                                  & -0.029$^{**}$  &                &                & -0.016$^{**}$  & -0.013$^{*}$\\   
                                                                                  & (0.013)        &                &                & (0.007)        & (0.007)\\   
         HTM Asset Share                                                          &                & -0.038$^{*}$   &                & -0.025         & -0.003\\   
                                                                                  &                & (0.021)        &                & (0.019)        & (0.006)\\   
         Unrealized HTM Losses / Tier 1 Capital                                   &                &                & -0.036$^{***}$ & -0.024$^{***}$ & 0.0008\\   
                                                                                  &                &                & (0.013)        & (0.005)        & (0.012)\\   
         Uninsured Deposit Share $\times$ HTM Asset Share                         &                &                &                &                & -0.021$^{**}$\\   
                                                                                  &                &                &                &                & (0.009)\\   
         Uninsured Deposit Share $\times$ Unrealized HTM Losses / Tier 1 Capital  &                &                &                &                & -0.016$^{*}$\\   
                                                                                  &                &                &                &                & (0.009)\\   
          \\
         Observations                                                             & 224            & 224            & 222            & 222            & 222\\  
         R$^2$                                                                    & 0.091          & 0.161          & 0.144          & 0.257          & 0.400\\  
         Adjusted R$^2$                                                           & 0.087          & 0.157          & 0.140          & 0.247          & 0.386\\  
         \bottomrule
      \end{tabular}
   \end{adjustbox}
\end{table}




==> figures/table4.tex <==

\begin{table}[htbp]
   \caption{\label{tab:liquid_assets} Cumulative returns correlated with liquid assets. This table reports estimated coefficients of regressions with the cumulative returns in excess of the S\&P 500 index for the banks in our sample from February 1, 2023 to March 17, 2023 as the outcome. \%
      In Column (1), we report the bivariate relationship with the liquid asset share (securities + cash scaled by total
   assets) measured in 2022q4. \%
      Column (2) adds uninsured deposit share to Column (1). \%
      Column (3) reports the coefficient with the cash scaled by total assets and securities scaled by total assets. \%
       Column (4) adds uninsured deposit share to Column (3). \%
       Column (5) interacts uninsured deposit share with cash and securities. \%
       All variables (except for the cumulative returns) are mean zero and standarized to have standard deviation one, prior to interactions.}
   \bigskip
   \centering
   \begin{adjustbox}{width = 1.2\textwidth, center}
      \begin{tabular}{lccccc}
         \toprule
                                                                     & (1)            & (2)            & (3)            & (4)            & (5)\\  
         \midrule 
         (Intercept)                                                 & -0.156$^{***}$ & -0.156$^{***}$ & -0.156$^{***}$ & -0.156$^{***}$ & -0.157$^{***}$\\   
                                                                     & (0.009)        & (0.009)        & (0.008)        & (0.008)        & (0.008)\\   
         Liquid Assets / Total Assets                                & -0.009         &                & 0.007          &                &   \\   
                                                                     & (0.012)        &                & (0.011)        &                &   \\   
         Cash / Total Assets                                         &                & 0.015$^{**}$   &                & 0.032$^{***}$  & 0.024$^{***}$\\   
                                                                     &                & (0.007)        &                & (0.009)        & (0.008)\\   
         Securities / Total Assets                                   &                & -0.020         &                & -0.008         & -0.005\\   
                                                                     &                & (0.013)        &                & (0.011)        & (0.008)\\   
         Uninsured Deposit Share                                     &                &                & -0.051$^{***}$ & -0.056$^{***}$ & -0.054$^{***}$\\   
                                                                     &                &                & (0.015)        & (0.015)        & (0.014)\\   
         Cash / Total Assets $\times$ Uninsured Deposit Share        &                &                &                &                & 0.015$^{**}$\\   
                                                                     &                &                &                &                & (0.007)\\   
         Securities / Total Assets $\times$ Uninsured Deposit Share  &                &                &                &                & -0.015\\   
                                                                     &                &                &                &                & (0.015)\\   
          \\
         Observations                                                & 224            & 224            & 224            & 224            & 224\\  
         R$^2$                                                       & 0.005          & 0.040          & 0.142          & 0.202          & 0.240\\  
         Adjusted R$^2$                                              & 0.0004         & 0.031          & 0.134          & 0.191          & 0.223\\  
         \bottomrule
      \end{tabular}
   \end{adjustbox}
\end{table}




==> figures/table4_beta.tex <==

\begin{table}[htbp]
   \caption{\label{tab:liquid_assets_beta} Cumulative returns correlated with liquid assets, adjusted for beta. This table reports estimated coefficients of regressions with the cumulative returns in excess of the S\&P 500 index, adjusted for beta estimated in 2002, for the banks in our sample from February 1, 2023 to March 17, 2023 as the outcome. \%
      In Column (1), we report the bivariate relationship with the liquid asset share (securities + cash scaled by total
   assets) measured in 2022q4. \%
      Column (2) adds uninsured deposit share to Column (1). \%
      Column (3) reports the coefficient with the cash scaled by total assets and securities scaled by total assets. \%
       Column (4) adds uninsured deposit share to Column (3). \%
       Column (5) interacts uninsured deposit share with cash and securities. \%
       All variables (except for the cumulative returns) are mean zero and standarized to have standard deviation one, prior to interactions.}
   \bigskip
   \centering
   \begin{adjustbox}{width = 1.2\textwidth, center}
      \begin{tabular}{lccccc}
         \toprule
                                                                     & (1)            & (2)            & (3)            & (4)            & (5)\\  
         \midrule 
         (Intercept)                                                 & -0.165$^{***}$ & -0.165$^{***}$ & -0.165$^{***}$ & -0.165$^{***}$ & -0.167$^{***}$\\   
                                                                     & (0.009)        & (0.009)        & (0.008)        & (0.008)        & (0.008)\\   
         Liquid Assets / Total Assets                                & -0.009         &                & 0.008          &                &   \\   
                                                                     & (0.012)        &                & (0.011)        &                &   \\   
         Cash / Total Assets                                         &                & 0.017$^{**}$   &                & 0.033$^{***}$  & 0.024$^{***}$\\   
                                                                     &                & (0.007)        &                & (0.010)        & (0.008)\\   
         Securities / Total Assets                                   &                & -0.021         &                & -0.009         & -0.005\\   
                                                                     &                & (0.014)        &                & (0.011)        & (0.008)\\   
         Uninsured Deposit Share                                     &                &                & -0.051$^{***}$ & -0.056$^{***}$ & -0.054$^{***}$\\   
                                                                     &                &                & (0.016)        & (0.016)        & (0.014)\\   
         Cash / Total Assets $\times$ Uninsured Deposit Share        &                &                &                &                & 0.016$^{**}$\\   
                                                                     &                &                &                &                & (0.007)\\   
         Securities / Total Assets $\times$ Uninsured Deposit Share  &                &                &                &                & -0.014\\   
                                                                     &                &                &                &                & (0.016)\\   
          \\
         Observations                                                & 224            & 224            & 224            & 224            & 224\\  
         R$^2$                                                       & 0.005          & 0.043          & 0.139          & 0.203          & 0.244\\  
         Adjusted R$^2$                                              & 0.0002         & 0.034          & 0.131          & 0.192          & 0.226\\  
         \bottomrule
      \end{tabular}
   \end{adjustbox}
\end{table}




==> figures/table4_late.tex <==

\begin{table}[htbp]
   \caption{\label{tab:liquid_assets_late} Cumulative returns correlated with liquid assets, long run. This table reports estimated coefficients of regressions with the cumulative returns in excess of the S\&P 500 index for the banks in our sample from February 1, 2023 to March 17, 2023 as the outcome. \%
      In Column (1), we report the bivariate relationship with the liquid asset share (securities + cash scaled by total
   assets) measured in 2022q4. \%
      Column (2) adds uninsured deposit share to Column (1). \%
      Column (3) reports the coefficient with the cash scaled by total assets and securities scaled by total assets. \%
       Column (4) adds uninsured deposit share to Column (3). \%
       Column (5) interacts uninsured deposit share with cash and securities. \%
       All variables (except for the cumulative returns) are mean zero and standarized to have standard deviation one, prior to interactions.}
   \bigskip
   \centering
   \begin{adjustbox}{width = 1.2\textwidth, center}
      \begin{tabular}{lccccc}
         \toprule
                                                                     & (1)            & (2)            & (3)            & (4)                   & (5)\\  
         \midrule 
         (Intercept)                                                 & -0.336$^{***}$ & -0.336$^{***}$ & -0.336$^{***}$ & -0.336$^{***}$        & -0.339$^{***}$\\   
                                                                     & (0.011)        & (0.011)        & (0.010)        & (0.010)               & (0.010)\\   
         Liquid Assets / Total Assets                                & 0.008          &                & 0.027$^{**}$   &                       &   \\   
                                                                     & (0.013)        &                & (0.012)        &                       &   \\   
         Cash / Total Assets                                         &                & 0.039$^{***}$  &                & 0.059$^{***}$         & 0.053$^{***}$\\   
                                                                     &                & (0.009)        &                & (0.011)               & (0.011)\\   
         Securities / Total Assets                                   &                & -0.014         &                & $9.36\times 10^{-5}$  & -0.002\\   
                                                                     &                & (0.013)        &                & (0.012)               & (0.009)\\   
         Uninsured Deposit Share                                     &                &                & -0.060$^{***}$ & -0.068$^{***}$        & -0.070$^{***}$\\   
                                                                     &                &                & (0.015)        & (0.015)               & (0.013)\\   
         Cash / Total Assets $\times$ Uninsured Deposit Share        &                &                &                &                       & 0.009\\   
                                                                     &                &                &                &                       & (0.008)\\   
         Securities / Total Assets $\times$ Uninsured Deposit Share  &                &                &                &                       & 0.002\\   
                                                                     &                &                &                &                       & (0.017)\\   
          \\
         Observations                                                & 224            & 224            & 224            & 224                   & 224\\  
         R$^2$                                                       & 0.002          & 0.068          & 0.122          & 0.218                 & 0.224\\  
         Adjusted R$^2$                                              & -0.002         & 0.059          & 0.114          & 0.208                 & 0.207\\  
         \bottomrule
      \end{tabular}
   \end{adjustbox}
\end{table}




==> figures/table4_late_beta.tex <==

\begin{table}[htbp]
   \caption{\label{tab:liquid_assets_late_beta} Cumulative returns correlated with liquid assets, adjusted for beta, long run. This table reports estimated coefficients of regressions with the cumulative returns in excess of the S\&P 500 index, adjusted for beta estimated in 2002, for the banks in our sample from February 1, 2023 to March 17, 2023 as the outcome. \%
      In Column (1), we report the bivariate relationship with the liquid asset share (securities + cash scaled by total
   assets) measured in 2022q4. \%
      Column (2) adds uninsured deposit share to Column (1). \%
      Column (3) reports the coefficient with the cash scaled by total assets and securities scaled by total assets. \%
       Column (4) adds uninsured deposit share to Column (3). \%
       Column (5) interacts uninsured deposit share with cash and securities. \%
       All variables (except for the cumulative returns) are mean zero and standarized to have standard deviation one, prior to interactions.}
   \bigskip
   \centering
   \begin{adjustbox}{width = 1.2\textwidth, center}
      \begin{tabular}{lccccc}
         \toprule
                                                                     & (1)            & (2)            & (3)            & (4)            & (5)\\  
         \midrule 
         (Intercept)                                                 & -0.321$^{***}$ & -0.321$^{***}$ & -0.321$^{***}$ & -0.321$^{***}$ & -0.324$^{***}$\\   
                                                                     & (0.011)        & (0.011)        & (0.010)        & (0.010)        & (0.010)\\   
         Liquid Assets / Total Assets                                & 0.008          &                & 0.027$^{**}$   &                &   \\   
                                                                     & (0.013)        &                & (0.012)        &                &   \\   
         Cash / Total Assets                                         &                & 0.039$^{***}$  &                & 0.059$^{***}$  & 0.053$^{***}$\\   
                                                                     &                & (0.009)        &                & (0.010)        & (0.011)\\   
         Securities / Total Assets                                   &                & -0.014         &                & 0.0001         & -0.002\\   
                                                                     &                & (0.013)        &                & (0.012)        & (0.009)\\   
         Uninsured Deposit Share                                     &                &                & -0.059$^{***}$ & -0.067$^{***}$ & -0.070$^{***}$\\   
                                                                     &                &                & (0.015)        & (0.015)        & (0.013)\\   
         Cash / Total Assets $\times$ Uninsured Deposit Share        &                &                &                &                & 0.009\\   
                                                                     &                &                &                &                & (0.008)\\   
         Securities / Total Assets $\times$ Uninsured Deposit Share  &                &                &                &                & 0.002\\   
                                                                     &                &                &                &                & (0.017)\\   
          \\
         Observations                                                & 224            & 224            & 224            & 224            & 224\\  
         R$^2$                                                       & 0.002          & 0.068          & 0.122          & 0.218          & 0.224\\  
         Adjusted R$^2$                                              & -0.002         & 0.059          & 0.114          & 0.207          & 0.206\\  
         \bottomrule
      \end{tabular}
   \end{adjustbox}
\end{table}




==> figures/table5.tex <==

\begin{table}[htbp]
   \caption{\label{tab:npl_capital} Cumulative returns correlated with NPL and Tier 1 capital. This table reports estimated coefficients of regressions with the cumulative returns in excess of the S\&P 500 index for the banks in our sample from February 1, 2023 to March 17, 2023 as the outcome. \%
      In Column (1), we report the bivariate relationship with the non-performing loan ratio (non-performing loans scaled by total loans) measured in 2022q4. \%
      Column (2) reports the coefficient with the the tier 1 capital ratio measured in 2022q4. \%
      Column (3) combines Column (1) and (2). \%
       Column (4) adds uninsured deposit share to Column (3). \%
       Column (5) interacts uninsured deposit share with non-performing loans and tier 1 capital. \%
       All variables (except for the cumulative returns) are mean zero and standarized to have standard deviation one, prior to interactions.}
   \bigskip
   \centering
   \begin{adjustbox}{width = 1.2\textwidth, center}
      \begin{tabular}{lccccc}
         \toprule
                                                                              & (1)            & (2)            & (3)            & (4)            & (5)\\  
         \midrule 
         (Intercept)                                                          & -0.159$^{***}$ & -0.156$^{***}$ & -0.159$^{***}$ & -0.158$^{***}$ & -0.151$^{***}$\\   
                                                                              & (0.009)        & (0.009)        & (0.009)        & (0.008)        & (0.009)\\   
         Tier 1 Capital Ratio                                                 & 0.032$^{***}$  &                & 0.032$^{***}$  & 0.022$^{**}$   & 0.036$^{*}$\\   
                                                                              & (0.011)        &                & (0.011)        & (0.011)        & (0.019)\\   
         Non-Performing Loans / Total Loans                                   &                & 0.003          & 0.0008         & -0.0003        & -0.004\\   
                                                                              &                & (0.009)        & (0.009)        & (0.008)        & (0.008)\\   
         Uninsured Deposit Share                                              &                &                &                & -0.047$^{***}$ & -0.049$^{***}$\\   
                                                                              &                &                &                & (0.017)        & (0.016)\\   
         Tier 1 Capital Ratio $\times$ Uninsured Deposit Share                &                &                &                &                & 0.032\\   
                                                                              &                &                &                &                & (0.024)\\   
         Non-Performing Loans / Total Loans $\times$ Uninsured Deposit Share  &                &                &                &                & 0.002\\   
                                                                              &                &                &                &                & (0.012)\\   
          \\
         Observations                                                         & 216            & 224            & 216            & 216            & 216\\  
         R$^2$                                                                & 0.060          & 0.0004         & 0.060          & 0.173          & 0.221\\  
         Adjusted R$^2$                                                       & 0.056          & -0.004         & 0.051          & 0.161          & 0.202\\  
         \bottomrule
      \end{tabular}
   \end{adjustbox}
\end{table}




==> figures/table5_beta.tex <==

\begin{table}[htbp]
   \caption{\label{tab:npl_capital_beta} Cumulative returns correlated with NPL and Tier 1 capital, adjusted for beta. This table reports estimated coefficients of regressions with the cumulative returns in excess of the S\&P 500 index, adjusted for beta estimated in 2002, for the banks in our sample from February 1, 2023 to March 17, 2023 as the outcome. \%
      In Column (1), we report the bivariate relationship with the non-performing loan ratio (non-performing loans scaled by total loans) measured in 2022q4. \%
      Column (2) reports the coefficient with the the tier 1 capital ratio measured in 2022q4. \%
      Column (3) combines Column (1) and (2). \%
       Column (4) adds uninsured deposit share to Column (3). \%
       Column (5) interacts uninsured deposit share with non-performing loans and tier 1 capital. \%
       All variables (except for the cumulative returns) are mean zero and standarized to have standard deviation one, prior to interactions.}
   \bigskip
   \centering
   \begin{adjustbox}{width = 1.2\textwidth, center}
      \begin{tabular}{lccccc}
         \toprule
                                                                              & (1)            & (2)            & (3)            & (4)            & (5)\\  
         \midrule 
         (Intercept)                                                          & -0.168$^{***}$ & -0.165$^{***}$ & -0.168$^{***}$ & -0.167$^{***}$ & -0.160$^{***}$\\   
                                                                              & (0.009)        & (0.009)        & (0.009)        & (0.008)        & (0.009)\\   
         Tier 1 Capital Ratio                                                 & 0.033$^{***}$  &                & 0.033$^{***}$  & 0.023$^{**}$   & 0.038$^{*}$\\   
                                                                              & (0.011)        &                & (0.011)        & (0.011)        & (0.020)\\   
         Non-Performing Loans / Total Loans                                   &                & 0.004          & 0.002          & 0.001          & -0.002\\   
                                                                              &                & (0.009)        & (0.009)        & (0.008)        & (0.008)\\   
         Uninsured Deposit Share                                              &                &                &                & -0.046$^{***}$ & -0.049$^{***}$\\   
                                                                              &                &                &                & (0.018)        & (0.017)\\   
         Tier 1 Capital Ratio $\times$ Uninsured Deposit Share                &                &                &                &                & 0.033\\   
                                                                              &                &                &                &                & (0.025)\\   
         Non-Performing Loans / Total Loans $\times$ Uninsured Deposit Share  &                &                &                &                & 0.002\\   
                                                                              &                &                &                &                & (0.012)\\   
          \\
         Observations                                                         & 216            & 224            & 216            & 216            & 216\\  
         R$^2$                                                                & 0.062          & 0.0009         & 0.063          & 0.171          & 0.222\\  
         Adjusted R$^2$                                                       & 0.058          & -0.004         & 0.054          & 0.159          & 0.203\\  
         \bottomrule
      \end{tabular}
   \end{adjustbox}
\end{table}




==> figures/table5_late.tex <==

\begin{table}[htbp]
   \caption{\label{tab:npl_capital_late} Cumulative returns correlated with NPL and Tier 1 capital, long run. This table reports estimated coefficients of regressions with the cumulative returns in excess of the S\&P 500 index for the banks in our sample from February 1, 2023 to May 10, 2023 as the outcome. \%
      In Column (1), we report the bivariate relationship with the non-performing loan ratio (non-performing loans scaled by total loans) measured in 2022q4. \%
      Column (2) reports the coefficient with the the tier 1 capital ratio measured in 2022q4. \%
      Column (3) combines Column (1) and (2). \%
       Column (4) adds uninsured deposit share to Column (3). \%
       Column (5) interacts uninsured deposit share with non-performing loans and tier 1 capital. \%
       All variables (except for the cumulative returns) are mean zero and standarized to have standard deviation one, prior to interactions.}
   \bigskip
   \centering
   \begin{adjustbox}{width = 1.2\textwidth, center}
      \begin{tabular}{lccccc}
         \toprule
                                                                              & (1)            & (2)            & (3)            & (4)            & (5)\\  
         \midrule 
         (Intercept)                                                          & -0.338$^{***}$ & -0.336$^{***}$ & -0.339$^{***}$ & -0.338$^{***}$ & -0.330$^{***}$\\   
                                                                              & (0.011)        & (0.011)        & (0.011)        & (0.010)        & (0.011)\\   
         Tier 1 Capital Ratio                                                 & 0.045$^{***}$  &                & 0.044$^{***}$  & 0.034$^{***}$  & 0.049$^{***}$\\   
                                                                              & (0.012)        &                & (0.012)        & (0.012)        & (0.018)\\   
         Non-Performing Loans / Total Loans                                   &                & 0.019$^{*}$    & 0.017          & 0.016          & 0.012\\   
                                                                              &                & (0.011)        & (0.011)        & (0.010)        & (0.009)\\   
         Uninsured Deposit Share                                              &                &                &                & -0.049$^{***}$ & -0.051$^{***}$\\   
                                                                              &                &                &                & (0.017)        & (0.016)\\   
         Tier 1 Capital Ratio $\times$ Uninsured Deposit Share                &                &                &                &                & 0.036$^{*}$\\   
                                                                              &                &                &                &                & (0.020)\\   
         Non-Performing Loans / Total Loans $\times$ Uninsured Deposit Share  &                &                &                &                & 0.003\\   
                                                                              &                &                &                &                & (0.013)\\   
          \\
         Observations                                                         & 216            & 224            & 216            & 216            & 216\\  
         R$^2$                                                                & 0.075          & 0.014          & 0.086          & 0.165          & 0.204\\  
         Adjusted R$^2$                                                       & 0.071          & 0.009          & 0.078          & 0.154          & 0.186\\  
         \bottomrule
      \end{tabular}
   \end{adjustbox}
\end{table}




==> figures/table5_late_beta.tex <==

\begin{table}[htbp]
   \caption{\label{tab:npl_capital_late_beta} Cumulative returns correlated with NPL and Tier 1 capital, adjusted for beta, long run. This table reports estimated coefficients of regressions with the cumulative returns in excess of the S\&P 500 index, adjusted for beta estimated in 2002, for the banks in our sample from February 1, 2023 to May 10, 2023 as the outcome. \%
      In Column (1), we report the bivariate relationship with the non-performing loan ratio (non-performing loans scaled by total loans) measured in 2022q4. \%
      Column (2) reports the coefficient with the the tier 1 capital ratio measured in 2022q4. \%
      Column (3) combines Column (1) and (2). \%
       Column (4) adds uninsured deposit share to Column (3). \%
       Column (5) interacts uninsured deposit share with non-performing loans and tier 1 capital. \%
       All variables (except for the cumulative returns) are mean zero and standarized to have standard deviation one, prior to interactions.}
   \bigskip
   \centering
   \begin{adjustbox}{width = 1.2\textwidth, center}
      \begin{tabular}{lccccc}
         \toprule
                                                                              & (1)            & (2)            & (3)            & (4)            & (5)\\  
         \midrule 
         (Intercept)                                                          & -0.324$^{***}$ & -0.321$^{***}$ & -0.324$^{***}$ & -0.323$^{***}$ & -0.315$^{***}$\\   
                                                                              & (0.011)        & (0.011)        & (0.011)        & (0.010)        & (0.011)\\   
         Tier 1 Capital Ratio                                                 & 0.045$^{***}$  &                & 0.043$^{***}$  & 0.033$^{***}$  & 0.049$^{***}$\\   
                                                                              & (0.012)        &                & (0.012)        & (0.012)        & (0.018)\\   
         Non-Performing Loans / Total Loans                                   &                & 0.019$^{*}$    & 0.017          & 0.016          & 0.012\\   
                                                                              &                & (0.011)        & (0.011)        & (0.010)        & (0.009)\\   
         Uninsured Deposit Share                                              &                &                &                & -0.049$^{***}$ & -0.051$^{***}$\\   
                                                                              &                &                &                & (0.017)        & (0.016)\\   
         Tier 1 Capital Ratio $\times$ Uninsured Deposit Share                &                &                &                &                & 0.035$^{*}$\\   
                                                                              &                &                &                &                & (0.020)\\   
         Non-Performing Loans / Total Loans $\times$ Uninsured Deposit Share  &                &                &                &                & 0.003\\   
                                                                              &                &                &                &                & (0.013)\\   
          \\
         Observations                                                         & 216            & 224            & 216            & 216            & 216\\  
         R$^2$                                                                & 0.075          & 0.013          & 0.086          & 0.165          & 0.204\\  
         Adjusted R$^2$                                                       & 0.071          & 0.009          & 0.077          & 0.153          & 0.185\\  
         \bottomrule
      \end{tabular}
   \end{adjustbox}
\end{table}




==> figures/table5_size.tex <==

\begin{table}[htbp]
   \caption{\label{tab:dep_assets} Cumulative returns correlated with asset size. This table reports estimated coefficients of regressions with the cumulative returns in excess of the S\&P 500 index for the banks in our sample. \%
      In Column (1), we report the relationship with binned indicator variables of total assets measured in 2022q4. The bins exhaustively bin out all observations, and do not include a constant, so each coefficient is the average for each bin. \%
      Column (2) includes the binned controls for assets (excluding the bin for banks with total assets less than 5 billion dollars) and a constant, as well as the controls for uninsured deposit share, tier 1 capital ratio, cash/ total assets and unrealized hold-to-maturity losses. Column 3 adds the cumulative abnormal return from February 1, 2022 to January 31, 2023 to Column (2). Columns (1)-(3) use cumluative returns from February 1, 2023 to March 17, 2023 as the outcome. Columns (4)-(6) repeat Columns (1)-(3) and use cumluative returns from February 1, 2023 to May 10, 2023 as the outcome.
       All variables (except for the cumulative returns) are mean zero and standarized to have standard deviation one, prior to interactions.}
   \bigskip
   \centering
   \begin{adjustbox}{width = 1.2\textwidth, center}
      \begin{tabular}{lcccccc}
         \toprule
                                                & (1)            & (2)            & (3)            & (4)            & (5)            & (6)\\  
         \midrule 
         Assets [0-5b]                          & -0.113$^{***}$ &                &                & -0.319$^{***}$ &                &   \\   
                                                & (0.009)        &                &                & (0.016)        &                &   \\   
         Assets (5b-10b]                        & -0.115$^{***}$ & 0.005          & 0.013          & -0.331$^{***}$ & 0.0005         & 0.008\\   
                                                & (0.010)        & (0.013)        & (0.013)        & (0.015)        & (0.022)        & (0.021)\\   
         Assets (10b-50b]                       & -0.160$^{***}$ & -0.034$^{**}$  & -0.035$^{**}$  & -0.354$^{***}$ & -0.014         & -0.015\\   
                                                & (0.013)        & (0.017)        & (0.015)        & (0.017)        & (0.025)        & (0.022)\\   
         Assets (50b-250b]                      & -0.314$^{***}$ & -0.169$^{***}$ & -0.150$^{***}$ & -0.375$^{***}$ & -0.019         & 0.0008\\   
                                                & (0.046)        & (0.028)        & (0.026)        & (0.060)        & (0.048)        & (0.050)\\   
         Assets (250b-1tr]                      & -0.224$^{***}$ & -0.102$^{***}$ & -0.078$^{**}$  & -0.333$^{***}$ & 0.011          & 0.036\\   
                                                & (0.026)        & (0.030)        & (0.030)        & (0.033)        & (0.045)        & (0.045)\\   
         Assets (1tr-10tr]                      & -0.122$^{***}$ & 0.018          & 0.029          & -0.148$^{***}$ & 0.211$^{***}$  & 0.223$^{***}$\\   
                                                & (0.016)        & (0.029)        & (0.030)        & (0.029)        & (0.046)        & (0.044)\\   
         (Intercept)                            &                & -0.127$^{***}$ & -0.140$^{***}$ &                & -0.338$^{***}$ & -0.352$^{***}$\\   
                                                &                & (0.011)        & (0.010)        &                & (0.018)        & (0.017)\\   
         Uninsured Deposit Share                &                & -0.037$^{***}$ & -0.026$^{**}$  &                & -0.066$^{***}$ & -0.053$^{***}$\\   
                                                &                & (0.013)        & (0.010)        &                & (0.014)        & (0.012)\\   
         Tier 1 Capital Ratio                   &                & 0.009          & 0.010          &                & 0.009          & 0.010\\   
                                                &                & (0.009)        & (0.008)        &                & (0.011)        & (0.011)\\   
         Cash / Total Assets                    &                & 0.036$^{***}$  & 0.022$^{**}$   &                & 0.054$^{***}$  & 0.039$^{***}$\\   
                                                &                & (0.009)        & (0.009)        &                & (0.011)        & (0.010)\\   
         Unrealized HTM Losses / Tier 1 Capital &                & -0.041$^{***}$ & -0.039$^{***}$ &                & -0.036$^{***}$ & -0.034$^{***}$\\   
                                                &                & (0.009)        & (0.007)        &                & (0.007)        & (0.007)\\   
         Cumulative Abnormal Returns (2022)     &                &                & 0.274$^{***}$  &                &                & 0.288$^{***}$\\   
                                                &                &                & (0.063)        &                &                & (0.095)\\   
          \\
         Observations                           & 224            & 216            & 216            & 224            & 216            & 216\\  
         R$^2$                                  & 0.242          & 0.522          & 0.606          & 0.045          & 0.350          & 0.409\\  
         Adjusted R$^2$                         & 0.225          & 0.502          & 0.587          & 0.023          & 0.321          & 0.380\\  
         \bottomrule
      \end{tabular}
   \end{adjustbox}
\end{table}




==> tables/regtable.tex <==

\begingroup
\centering
\begin{tabular}{lcccc}
   \toprule
   Dependent Variable: & \multicolumn{4}{c}{Cumulative Returns from March 1-13, 2023}\\
                                  & (1)             & (2)             & (3)            & (4)\\  
   \midrule
   (Intercept)                             & 0.0190          & -0.1296$^{***}$ & 0.0165         & -0.0386\\   
                                           & (0.0579)        & (0.0266)        & (0.0561)       & (0.0642)\\   
   Uninsured Share of Deposits                        & -0.4639$^{***}$ &                 & -0.4303$^{**}$ & -0.3096\\   
                                           & (0.1670)        &                 & (0.1647)       & (0.2019)\\   
   Hold-to-Maturity Share of Assets                             &                 & -0.6189         & -0.1630        & 0.6337\\   
                                           &                 & (0.4091)        & (0.3656)       & (0.6567)\\   
   Uninsured Share $\times$ Hold-to-Maturity Share    &                 &                 &                & -1.404\\   
                                           &                 &                 &                & (1.456)\\   
   \midrule
   \emph{Fit statistics}\\
   Observations                            & 93              & 93              & 93             & 93\\  
   R$^2$                                   & 0.24853         & 0.08609         & 0.25320        & 0.27789\\  
   Adjusted R$^2$                          & 0.24027         & 0.07605         & 0.23660        & 0.25355\\  
   \bottomrule
\end{tabular}
\par\endgroup




==> tables/table1_fdic.tex <==
\begin{table}[!htbp] \centering \renewcommand*{\arraystretch}{1.1}\caption{Summary Statistics}\resizebox{\textwidth}{!}{
\begin{tabular}{lrrrr}
\hline
\hline
Variable & NotNA & Mean & Median & Sd \\ 
\hline
FDIC Assets (000) & 221 & 84524180 & 10777878 & 325,733,797 \\ 
Uninsured Deposit Share & 221 & 39\% & 38\% & 18\%\\ 
\hline
\hline
\end{tabular}
}
\end{table}



==> tables/table1_y9c.tex <==
\begin{table}[!htbp] \centering \renewcommand*{\arraystretch}{1.1}\caption{Summary Statistics}\resizebox{\textwidth}{!}{
\begin{tabular}{lrrrr}
\hline
\hline
Variable & NotNA & Mean & Median & Sd \\ 
\hline
Assets (000) & 224 & 101688402 & 9559211 & 405,970,115 \\ 
Cash / Assets & 224 & 9.2\% & 8.1\% & 7\% \\ 
Securities / Assets & 224 & 20\% & 18\% & 11\% \\ 
Liquid Assets / Assets & 224 & 29\% & 27\% & 13\% \\ 
Unrealized HTM Losses / Tier 1 Capital & 222 & 0.21\% & 0\% & 2.2\% \\ 
Hold-to-Maturity Securities / Assets & 224 & 3.2\% & 0.33\% & 5.9\% \\ 
Unisured Deposit Share & 224 & 39\% & 38\% & 18\% \\ 
Tier 1 Capital Ratio & 216 & 13\% & 12\% & 2.9\%\\ 
\hline
\hline
\end{tabular}
}
\end{table}



==> tables/table2.tex <==
\begin{table}[!htbp] \centering \renewcommand*{\arraystretch}{1.1}\caption{Summary Statistics}\resizebox{\textwidth}{!}{
\begin{tabular}{lrrrrrrr}
\hline
\hline
Variable & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{SD} & \multicolumn{1}{c}{5th Pct.} & \multicolumn{1}{c}{25th Pct.} & \multicolumn{1}{c}{50th Pct.} & \multicolumn{1}{c}{75th Pct.} & \multicolumn{1}{c}{95th Pct.} \\ 
\hline
\multicolumn{8}{c}{Date: 2023-01-31} \\ 
Cumulative Abnormal Returns & 2.9\% & 15\% & -25\% & -5.7\% & 3.7\% & 12\% & 27\% \\ 
 &  &  &  &  &  &  &  \\ 
\multicolumn{8}{c}{Date: 2023-03-17} \\ 
Cumulative Abnormal Returns & -16\% & 13\% & -35\% & -18\% & -14\% & -8.2\% & -2.6\% \\ 
 &  &  &  &  &  &  &  \\ 
\multicolumn{8}{c}{Date: 2023-05-25} \\ 
Cumulative Abnormal Returns & -30\% & 16\% & -51\% & -38\% & -29\% & -22\% & -9.9\%\\ 
\hline
\hline
\end{tabular}
}
\end{table}



==> tables/table3_short.tex <==

\begin{table}[htbp]
   \caption{\label{tab:dep_htm_short} Cumulative returns correlated with uninsured deposits and HTM, immediately after SVB shutdown. This table reports estimated coefficients of regressions with the cumulative returns in excess of the S\&P 500 index for the banks in our sample from February 1, 2023 to March 10, 2023 as the outcome.  In Column (1), we report the bivariate relationship with the uninsured deposit share (uninsured deposts as a share of total
   deposits) measured in 2022q4. Column (2) reports the coefficient with the hold-to-maturity asset share (hold-to-maturity assets
   as a share of total assets) measured in 2022q4. Column (3) reports unrealized hold-to-
   maturity losses scaled by tier 1 capital. Column (4) combines Columns (1)-(3). Column (5) adds the interaction of uninsured deposit share with HTM Asset Share and Unrealized HTM Losses. All variables (except for the cumulative returns) are mean zero and standarized to have standard deviation one, prior to interactions.}
   \bigskip
   \centering
   \begin{adjustbox}{width = 1.2\textwidth, center}
      \begin{tabular}{lccccc}
         \toprule
                                                                                  & (1)            & (2)            & (3)            & (4)            & (5)\\  
         \midrule 
         Constant                                                                 & -0.071$^{***}$ & -0.071$^{***}$ & -0.071$^{***}$ & -0.071$^{***}$ & -0.061$^{***}$\\   
                                                                                  & (0.006)        & (0.006)        & (0.006)        & (0.005)        & (0.005)\\   
         Uninsured Deposit Share                                                  & -0.029$^{**}$  &                &                & -0.016$^{**}$  & -0.013$^{*}$\\   
                                                                                  & (0.013)        &                &                & (0.007)        & (0.007)\\   
         HTM Asset Share                                                          &                & -0.038$^{*}$   &                & -0.025         & -0.003\\   
                                                                                  &                & (0.021)        &                & (0.019)        & (0.006)\\   
         Unrealized HTM Losses / Tier 1 Capital                                   &                &                & -0.036$^{***}$ & -0.024$^{***}$ & 0.0008\\   
                                                                                  &                &                & (0.013)        & (0.005)        & (0.012)\\   
         Uninsured Deposit Share $\times$ HTM Asset Share                         &                &                &                &                & -0.021$^{**}$\\   
                                                                                  &                &                &                &                & (0.009)\\   
         Uninsured Deposit Share $\times$ Unrealized HTM Losses / Tier 1 Capital  &                &                &                &                & -0.016$^{*}$\\   
                                                                                  &                &                &                &                & (0.009)\\   
          \\
         Observations                                                             & 224            & 224            & 222            & 222            & 222\\  
         R$^2$                                                                    & 0.091          & 0.161          & 0.144          & 0.257          & 0.400\\  
         Adjusted R$^2$                                                           & 0.087          & 0.157          & 0.140          & 0.247          & 0.386\\  
         \bottomrule
      \end{tabular}
   \end{adjustbox}
\end{table}




==> tables/table5_size_beta.tex <==

\begin{table}[htbp]
   \caption{\label{tab:dep_assets_beta} Cumulative returns correlated with asset size, adjusted for beta. This table reports estimated coefficients of regressions with the cumulative returns in excess of the S\&P 500 index, adjusted for beta estimated in 2002, for the banks in our sample. \%
      In Column (1), we report the relationship with binned indicator variables of total assets measured in 2022q4. The bins exhaustively bin out all observations, and do not include a constant, so each coefficient is the average for each bin. \%
      Column (2) includes the binned controls for assets (excluding the bin for banks with total assets less than 5 billion dollars) and a constant, as well as the controls for uninsured deposit share, tier 1 capital ratio, cash/ total assets and unrealized hold-to-maturity losses. Column 3 adds the cumulative abnormal return from February 1, 2022 to January 31, 2023 to Column (2). Columns (1)-(3) use cumluative returns from February 1, 2023 to March 17, 2023 as the outcome. Columns (4)-(6) repeat Columns (1)-(3) and use cumluative returns from February 1, 2023 to May 25, 2023 as the outcome.
       All variables (except for the cumulative returns) are mean zero and standarized to have standard deviation one, prior to interactions.}
   \bigskip
   \centering
   \begin{adjustbox}{width = 1.2\textwidth, center}
      \begin{tabular}{lcccccc}
         \toprule
                                                & (1)            & (2)            & (3)            & (4)            & (5)            & (6)\\  
         \midrule 
         Assets [0-5b]                          & -0.131$^{***}$ &                &                & -0.274$^{***}$ &                &   \\   
                                                & (0.008)        &                &                & (0.015)        &                &   \\   
         Assets (5b-10b]                        & -0.126$^{***}$ & 0.013          & 0.020          & -0.270$^{***}$ & 0.015          & 0.022\\   
                                                & (0.010)        & (0.014)        & (0.013)        & (0.015)        & (0.023)        & (0.021)\\   
         Assets (10b-50b]                       & -0.166$^{***}$ & -0.021         & -0.022         & -0.301$^{***}$ & -0.005         & -0.006\\   
                                                & (0.013)        & (0.017)        & (0.015)        & (0.017)        & (0.024)        & (0.022)\\   
         Assets (50b-250b]                      & -0.317$^{***}$ & -0.152$^{***}$ & -0.134$^{***}$ & -0.318$^{***}$ & -0.002         & 0.015\\   
                                                & (0.048)        & (0.029)        & (0.027)        & (0.063)        & (0.050)        & (0.051)\\   
         Assets (250b-1tr]                      & -0.223$^{***}$ & -0.080$^{**}$  & -0.057$^{*}$   & -0.278$^{***}$ & 0.026          & 0.049\\   
                                                & (0.028)        & (0.032)        & (0.033)        & (0.030)        & (0.041)        & (0.041)\\   
         Assets (1tr-10tr]                      & -0.118$^{***}$ & 0.042          & 0.052$^{*}$    & -0.133$^{***}$ & 0.186$^{***}$  & 0.196$^{***}$\\   
                                                & (0.017)        & (0.030)        & (0.031)        & (0.024)        & (0.039)        & (0.039)\\   
         Constant                               &                & -0.145$^{***}$ & -0.158$^{***}$ &                & -0.294$^{***}$ & -0.306$^{***}$\\   
                                                &                & (0.011)        & (0.010)        &                & (0.018)        & (0.017)\\   
         Uninsured Deposit Share                &                & -0.039$^{***}$ & -0.028$^{**}$  &                & -0.064$^{***}$ & -0.053$^{***}$\\   
                                                &                & (0.013)        & (0.011)        &                & (0.014)        & (0.013)\\   
         Tier 1 Capital Ratio                   &                & 0.008          & 0.009          &                & 0.007          & 0.008\\   
                                                &                & (0.009)        & (0.008)        &                & (0.011)        & (0.010)\\   
         Cash / Total Assets                    &                & 0.037$^{***}$  & 0.023$^{***}$  &                & 0.047$^{***}$  & 0.034$^{***}$\\   
                                                &                & (0.010)        & (0.009)        &                & (0.011)        & (0.010)\\   
         Unrealized HTM Losses / Tier 1 Capital &                & -0.043$^{***}$ & -0.041$^{***}$ &                & -0.039$^{***}$ & -0.037$^{***}$\\   
                                                &                & (0.010)        & (0.008)        &                & (0.008)        & (0.008)\\   
         Cumulative Abnormal Returns (2022)     &                &                & 0.260$^{***}$  &                &                & 0.257$^{**}$\\   
                                                &                &                & (0.067)        &                &                & (0.102)\\   
          \\
         Observations                           & 224            & 216            & 216            & 224            & 216            & 216\\  
         R$^2$                                  & 0.211          & 0.509          & 0.583          & 0.031          & 0.314          & 0.361\\  
         Adjusted R$^2$                         & 0.193          & 0.487          & 0.562          & 0.009          & 0.284          & 0.330\\  
         \bottomrule
      \end{tabular}
   \end{adjustbox}
\end{table}



